Learning Bill Similarity with Annotated and Augmented Corpora of Bills

Bill writing is a critical element of representative democracy. However, it is often overlooked that most legislative bills are derived, or even directly copied, from other bills. Despite the significance of bill-to-bill linkages for understanding the legislative process, existing approaches fail to address semantic similarities across bills, let alone reordering or paraphrasing which are prevalent in legal document writing. In this paper, we overcome these limitations by proposing a 5-class classification task that closely reflects the nature of the bill generation process. In doing so, we construct a human-labeled dataset of 4,721 bill-to-bill relationships at the subsection-level and release this annotated dataset to the research community. To augment the dataset, we generate synthetic data with varying degrees of similarity, mimicking the complex bill writing process. We use BERT variants and apply multi-stage training, sequentially fine-tuning our models with synthetic and human-labeled datasets. We find that the predictive performance significantly improves when training with both human-labeled and synthetic data. Finally, we apply our trained model to infer section- and bill-level similarities. Our analysis shows that the proposed methodology successfully captures the similarities across legal documents at various levels of aggregation.

==> extra_annotation_experiment.tex <==
\add{The similarity distribution of subsection pairs is highly skewed, i.e., it is rare to observe that any random subsection pairs are related. We choose the 0.85 threshold to reflect the skewed distribution after examining sample pairs across all similarity ranges. To verify whether our model performs outside of the similarity range, we conduct an extra experiment by randomly sampling 2,468 pairs with similarity scores less than 0.85. As expected, our model predicts most of the pairs as \textit{Unrelated}.
\begin{itemize}
\item \textit{Unrelated}: 98.87\% (2,440 pairs) 
\item \textit{Partially Related}: 1.01\% (25 pairs) 
\item \textit{Related}: 0.12\% (3 pairs)
\end{itemize}
Furthermore, we annotate additional 213 pairs that are randomly sampled from these 2,468 pairs, including the pairs predicted as \textit{Related} or \textit{Partially Related}. All pairs are judged by annotators to be \textit{Unrelated}, except for two boilerplate pairs. This result shows that our model works on pairs with all similarity range.}

